From Compliant to Rigid Contact Simulation: a Unified and Efficient Approach

Whether rigid or compliant, contact interactions are inherent to robot motions, enabling them to move or manipulate things. Contact interactions result from complex physical phenomena, that can be mathematically cast as Nonlinear Complementarity Problems (NCPs) in the context of rigid or compliant point contact interactions. Such a class of complementarity problems is, in general, difficult to solve both from an optimization and numerical perspective. Over the past decades, dedicated and specialized contact solvers, implemented in modern robotics simulators (e.g., Bullet, Drake, MuJoCo, DART, Raisim) have emerged. Yet, most of these solvers tend either to solve a relaxed formulation of the original contact problems (at the price of physical inconsistencies) or to scale poorly with the problem dimension or its numerical conditioning (e.g., a robotic hand manipulating a paper sheet). In this paper, we introduce a unified and efficient approach to solving NCPs in the context of contact simulation. It relies on a sound combination of the Alternating Direction Method of Multipliers (ADMM) and proximal algorithms to account for both compliant and rigid contact interfaces in a unified way. To handle ill-conditioned problems and accelerate the convergence rate, we also propose an efficient update strategy to adapt the ADMM hyperparameters automatically. By leveraging proximal methods, we also propose new algorithmic solutions to efficiently evaluate the inverse dynamics involving rigid and compliant contact interactions, extending the approach developed in MuJoCo. We validate the efficiency and robustness of our contact solver against several alternative contact methods of the literature and benchmark them on various robotics and granular mechanics scenarios. Our code is made open-source at https://github.com/Simple-Robotics/Simple.

==> reviews/area-chair-2FCK.tex <==
\section{General comment and Meta Review}

\subsection{General comment}

The authors warmly thank the Area Chair and the reviewers for the work they did by providing detailed reviews.
We believe the quality of the reviews helped to improve the manuscript.
The main new contributions of the revised version are:
\begin{itemize}
    \item we provide a benchmark of our approach against state-of-the-art simulators e.g. MuJoCo and Drake;
    \item we discuss the differences between our approach and the one from \cite{tasora2021solving} in section II.F;
    \item we added an ablation study on the adaptive setting of the $\rho$ parameter between linear and spectral strategies;
    \item we demonstrate the ability of our approach to simulate compliant contacts;
    \item we updated the video of the supplementary materials to illustrate the benchmarks against other physics engines, the ability to handle both rigid and compliant contacts, and the benefits of using the spectral update rule for the proximal parameter.
\end{itemize}
Below we provide answers to the comments from the reviewers in their order of appearance.
In addition, a PDF document highlighting the changes made to the manuscript and the updated manuscript are attached to this letter.


\subsection{Meta Review by Area Chair 2FCK}

\noindent
\noindent
{\color{blue}\textbf{A.C.}} \citrev{The biggest complaint among the reviewers is that the authors do not compare to other state-of-the-art methods (even those repeatedly mentioned in the paper), especially MuJoCo and Drake.}

\noindent
\response We thank the Area Chair and the reviewers for their interesting remarks on the performance comparisons between physics engines.
Our paper compares contact solvers (and their underlying contact modeling) rather than the simulators directly. This would involve many more components (rigid body algorithms, collision detection algorithms, etc.).
Even if simulators like MuJoCo, Drake, or Bullet are open-source, their contact solvers are often intricate with a complete simulation pipeline.
For this reason, contact solvers are rarely exposed to the user, making it very difficult to use them as "off-the-shelf" solvers and compare them fairly with our solver.
Yet, we have incorporated our ADMM-based contact solvers inside a homemade simulation loop, which includes collision detection and contact solving. 
In the revised paper, we measure the performance of our approach against state-of-the-art simulators, MuJoCo, Drake, and Bullet, in terms of the number of simulation steps per second.
We demonstrate that our approach achieves simulation rates that are competitive with these simulators even though we did not relax any physical principles.
The benchmark is incorporated in section V of the paper.
This is a preliminary benchmark, but we believe the robotics community would benefit from a more in-depth comparison of simulation tools involving real experiments. 
Please check the supplementary material video for an illustration of this point.\\


\noindent
{\color{blue}\textbf{A.C.}} \citrev{One reviewer points out a very similar ADMM-based contact simulation paper that the authors may have been unaware of.}


\noindent
\response We agree with the Area Chair and reviewer Qz61 that the paper \cite{tasora2021solving} is related to our work and should be reviewed in the literature review.
As mentioned by the reviewer, the paper \cite{tasora2021solving} proposes to use an ADMM approach for contact simulation.
However, the approach from this work significantly differs from ours on both the modeling and algorithmic aspects.
Indeed, \cite{tasora2021solving} uses a CCP formulation, which results in an approximate Signorini condition~\cite{lelidec2023contact}, while we directly tackle the NCP problem.
In addition, for their ADMM algorithm, \cite{tasora2021solving} uses a proximal parameter update factor based on the ratio of primal and dual residuals, which changes at each iteration of the ADMM loop, thus requiring a new costly matrix inversion or decomposition. 
In our approach, we use an update factor strategy based on the condition number of $G$ which makes the algorithm more robust with respect to the conditioning of the problem.
Additionally, in their internal ADMM loop, they solve an ADMM problem involving both primal (joint velocities) and dual (constraint forces) variables, leading to the solving of a system of equations larger than ours.
In the revised version of the paper, we mention this work in section II.F "Existing solvers" when discussing CCP solvers.

==> reviews/reviewers/reviewer-Qz61.tex <==
\section{Reviewer Qz61}

\subsection{Summary of limitations}

\noindent
\reviewer{3.1} \citrev{The experiments themselves are somewhat limited lack thoroughness.
The only comparison in the paper is to vanilla PGS, and it is unclear why this was chosen as the baseline.
The paper repeatedly refers to MuJoCo and Drake as natural reference points, calling them "the closest to our work."
Given that both of these simulators are open source, it seems natural that they would, instead, be used.
Since both simulators use a convex approximation, I would not expect the presented work to be faster.
However, I would encourage authors to find experiments which demonstrate that they achieve a performant blend of speed and accuracy, when compared to the current state-of-the-art.}

\noindent
\response Please see our answer to the Area Chair comment for more details on this point.

\noindent
\reviewer{3.2} \citrev{The paper places an emphasis on the update rule for the ADMM parameter rho, highlighting that frequent changes are undesirable due the need to refactorize the Delassus matrix.
However, no evidence is provided to support the value of this contribution.
Ablation studies are needed to demonstrate that this spectral update rule does notably improve performance against the classical linear approach, across a range of possible increment/decrement factors.}

\noindent
\response We thank the reviewer for the nice suggestion.
In the revised paper, we provide an ablation study on the adaptive setting of the $\rho$ parameter on the convergence rates from Fig. 3.
The modified figure demonstrates the spectral update rule does notably improve performance against the classical linear approach on both the simulation of Talos robot and the wall of cubes. 
We also provide a comparative study over different values of $\tau$ and $p$ parameters associated with the linear and spectral update strategies on the set of benchmarking problems identified by the computational mechanics community. 
This study is reported in Sec V.C and summarized in Tab.III in the revised version of the paper. 
This study shows that the spectral strategy results in a lower number of Cholesky updates (the most costly operation in the ADMM solver) and more consistent statistics over the set of problems considered.
Please check the video of the supplementary material for an illustration of this point.

\noindent
\reviewer{3.3} \citrev{There is a recent paper, which uses a very similar ADMM formulation to simulate contact dynamics [a].
In fact, the ADMM partition is essentially identical: a linear solve followed by projection onto the friction cone. While there may be key differences between this existing paper and the submitted one, it seems that the authors are not familiar with this paper, as it was not cited.
It is imperative that a rebuttal address these similarities, and identify whatever novel contributions exist in the current submission.}

\noindent
\response Please see our response to the Area Chair's comment for more details on this point.



\subsection{Feedback For Improvement Or Clarification:}




\noindent
\reviewer{3.4} \citrev{The introduction of compliant contact in II-B should clearly state that this is, essentially, the simplest possible model of soft contact (linear elasticity), but that many alternatives exist which better capture the complex mechanics of deformable bodies.}

\noindent
\response We thank the reviewer for this suggestion.
In the revised manuscript, we mention more involved compliant contact models based on Finite Element Methods in section II.E "unilateral contact hypothesis" and cite some related works \cite{reddy1993introduction,ma2019dense}.


\noindent
\reviewer{3.5} \citrev{ The index reduction used in (23) and (24) seems to assume that contact is currently established (phi=0). Would it not be simpler to add $\Phi(q_k)$ to the right hand side?}

\noindent
\response We thank the reviewer for this nice remark.
Indeed (23) and (24) assume $\Phi(q^t)$ to be included in $\gamma$.
This was not clear in the original manuscript and we clarify this in the revised paper just after Eq. (23).



\noindent
\reviewer{3.6} \citrev{Equation (26) introduces the variable $c^(i)$ without definition.}

\noindent
\response c corresponds to the contact point velocity and was defined after equation (23). 
However, this may be unclear at this stage of the paper so we recall it in the revised paper.


\noindent
\reviewer{3.7} \citrev{The paper cites two works [23] and [31] which discuss some of the tradeoffs between contact models, but neither of these papers address physical experiments.
I would, suggest also reviewing papers which attempt to validate contact models on real-world data.}

\noindent
\response Indeed, [23] and [31] discuss contact model hypotheses, their implementation, and their impact on the simulation results, but no validation on real-world data is provided.
In the revised paper, we mention the works \cite{fazeli2017empirical,acosta2022validating} comparing simulators to real experiments. 




==> reviews/reviewers/reviewer-Tcne.tex <==
\section{Reviewer Tcne}

\subsection{Summary of limitations}

\noindent
\reviewer{2.1} \citrev{ First, the results do not compare with state-of-the-art engines like MuJoCo IsaacSim/PhysX, Drake, Raisim, etc.}

\noindent
\response Please see our response to the Area Chair's comment for more details on this point.

\noindent
\reviewer{2.2} \citrev{ Second, one of the most important recent trends for robot physics engines is implementation for accelerators (eg, MuJoCo XLA/MJX and IsaacGym) to enable high throughput for reinforcement learning.
This work does not discuss the potential performance or complexity results of the proposed methods for hardware like GPUs. 
}

\noindent
\response  As mentioned by the reviewer, a recent trend in physics engines is to implement them on hardware accelerators to enable high throughput for reinforcement learning.
This research direction is not the focus of this work, which aims at efficient simulation that can be performed online on an embedded system.
However, such acceleration via parallelization was added in a second stage of development for simulators like MuJoCo and PhysX, and we consider this an exciting future work for our algorithm.
At first glance, we do not foresee any particular limitations of implementing our approach on hardware accelerators, in the similar spirit of the transition that occurs between MuJoCo and MJX.
We added a comment on this recent trend in the discussion section.


\noindent
\reviewer{2.3} \citrev{Third, the theoretical results from the paper are nice, but it is not clear if there are significant practical advantages to the proposed algorithm compared to existing physics engines that have been developed over a number of years.}

\noindent
\response We thank the reviewer for pointing out our lack of clarity on the potential practical benefits of our approach.
Our work builds on previous works \cite{horak2019similarities,lelidec2023contact} demonstrating the simulation artifacts introduced by the contact models and algorithms of the current physics engines.
Our approach proposes to tighten the reality gap by solving the NCP robustly via an ADMM algorithm.
However, evaluating the benefits of a reduced reality gap on downstream tasks like control or reinforcement learning is an interesting research direction and would require its dedicated study.
In addition, please see our answer to the Area Chair's comment for more details on the performance comparison with other existing physics engines.
Please also see the updated supplementary material, in which we illustrate the importance of solving the NCP without any relaxation.
In the revised paper, we have added a comment on the potential practical advantages of our approach in the discussion section.


\subsection{Feedback For Improvement Or Clarification:}


\noindent
\reviewer{2.4} \citrev{The characterizations of Drake utilizing an LCP or MuJoCo-style contact model throughout the paper are incorrect.
Please see: \url{https://drake.mit.edu/doxygen_cxx/group__drake__contacts.html}}

\noindent
\response As introduced in \cite{castro2022unconstrained}, Drake uses a CCP contact model and a Newton solver which is similar to what is done in MuJoCo.

\noindent
\reviewer{2.5} \citrev{The abstract uses the term “punctual”.
The meaning of this term is unclear.}

\noindent
\response We thank the reviewer for indicating this wrong wording.
We corrected this in the revised version.

\noindent
\reviewer{2.6} \citrev{Section II A. Please comment on why Eq 5 may not be invertible (eg, M poorly conditioned, Jc rank deficient)}

\noindent
\response We thank the reviewer for reporting this lack of explanation.
In the revised version, we specify that the system may not be invertible due to the rank deficiency of the contact Jacobian.

\noindent
\reviewer{2.7} \citrev{Section II B “R being positive semi-definite makes the system (8)”: should be positive-definite otherwise the case R=0 is possible and the system may not be invertible}

\noindent
\response We thank the reviewer for pointing out this mistake.
We corrected this in the revised version.

\noindent
\reviewer{2.8} \citrev{Section F. Existing solvers: Bullet has a nonlinear friction cone, for example see Erwin's comment: \url{https://pybullet.org/Bullet/phpBB3/viewtopic.php?t=12500}}

\noindent
\response As mentioned by the reviewer, the current version of Bullet includes second-order friction cones for the contact model.
We modified the text to reflect this information, and, in particular, we updated table 1.

\noindent
\reviewer{2.9} \citrev{Nonlinear complementarity problem section reference equation should give a number, not (NCP)}

\noindent
\response We corrected this in the revised version. 

\noindent
\reviewer{2.10} \citrev{Section III A uses the term “Quadratically Constrained Quadratic Program”.
Isn't 27a a convex second-order cone program?
It's only a QCQP if you square the friction cone constraint-the paper doesn't mention performing this operation.
Additionally, QCQP implies that the problem may be non-convex and potentially challenging to solve without heuristics.}

\noindent
\response The problem (28a) has a second-order cone constraint and a quadratic cost function which makes it a Quadratically Constrained Quadratic Program.
Both the constraint and the cost function are convex which makes the problem convex.
As mentioned by the reviewer, the QCQP formulation could be written as a SOCP by rewriting the quadratic part of the cost function as a second-order cone constraint.
However, this operation is avoided here as it would require performing a Cholesky factorization of the Hessian matrix $G$ which is computationally expensive.
Moreover, this QCQP can be solved efficiently via the ADMM algorithm detailed in the paper.

\noindent
\reviewer{2.11} \citrev{Section IV: include complexity analysis comparison between the forward dynamics and inverse dynamics using the specialized analytical solution.
Additionally, the MuJoCo inverse dynamics can be decomposed by contact, please comment on their formulation and the proposed algorithm's inverse dynamics.}

\noindent
\response Our formulation can also be decomposed by contact.
It is actually close to the one of MuJoCo, the main difference being the additional de Saxce corrective term and the proximal term necessary for pure rigid contact interactions.
Thus leading to a computational complexity similar to the one of MuJoCo.

\noindent
\reviewer{2.12} \citrev{The proposed algorithm is compared with PGS and SCS.
Please compare with another engine, for example: MuJoCo or Raisim.
Further, a more compelling comparison would be to replicate the experiments from \url{https://homes.cs.washington.edu/~todorov/papers/ErezICRA15.pdf} or \url{https://homes.cs.washington.edu/~todorov/papers/TodorovICRA14.pdf}}


\noindent
\response  Please see our response to the Area Chair's comment for more details on this point.

\noindent
\reviewer{2.13} \citrev{Today many physics engines are implemented on accelerators (eg, Isaac Gym/PhysX, MJX/MuJoCo) to enable high throughput for RL.
Please comment on how the proposed algorithm would perform in this setting.
For example, the algorithm requires many iterations which may be less performant on GPU}

\noindent
\response As shown by Fig.3, in general, our algorithm requires fewer iterations than  PGS-like approaches to converge towards the solution of the NCP problem.
However, it would still require an additional effort to efficiently implement in a GPU framework the operations involved in ADMM and we leave this as future work. 
Please see R.2.2 for more details on the links between our work and the ongoing developments of simulation on GPUs.

\noindent
\reviewer{2.14} \citrev{Please comment on the frequency of collision detection calls.
Is this routine called at each ADMM iteration?
If so, this makes the proposed algorithm very expensive.}

\noindent
\response We thank the reviewer for indicating this lack of thoroughness.
We avoid calling the collision detection routine at each ADMM iteration by choosing an Euler explicit integration scheme.
We added a comment on this after introducing the integration scheme in Equation 22 of the revised version.

\noindent
\reviewer{2.15} \citrev{The examples do not demonstrate the compliant contact model.
A reader would expect to see how the simulation changes as compliance is increased/decreased.
Perhaps add a sphere dropping on a flat surface for different amounts of compliance.}


\noindent
\response We thank the reviewer for this suggestion.
In the original manuscript, we focused on the rigid case as it is more computationally challenging.
However, our approach can handle compliant contacts, so we added screenshots demonstrating compliant simulation on a humanoid (Fig.2 of revised paper) and a video sample in the supplementary material.

\noindent
\reviewer{2.16} \citrev{The term “hyper-static” is used without definition.}


\noindent
\response We thank the reviewer for reporting this omission.
In the revised paper, we specify that hyperstatic systems correspond to the case when $J_c$ is rank deficient.

\noindent
\reviewer{2.17} \citrev{In Section V Convergence analysis section, please report the condition number and indicate the value where the proposed algorithm fails (eg, does a playing card interacting with a very massive object fail?).}


\noindent
\response We thank the reviewer for this nice suggestion.
The two scenarios considered for the convergence analysis are a wall of cubes and the Talos robot.
In both cases, the problem is hyperstatic so the Delassus matrix exhibits null eigenvalues.
However, these two problems differ by the mass ratios they involve: this ratio is of $10^4$ for the wall of cubes and $10^1$ for the Talos scenario.
We provide this information in the revised paper.

\noindent
\reviewer{2.18} \citrev{What are the limits of ill conditioning? 
Usually ADMM is sensitive to this property.}


\noindent
\response As mentioned by the reviewer, ADMM is sensitive to the conditioning of the problem.
However, our approach which sets the proximal parameter adaptively via a spectral rule is able to mitigate this issue and solve ill-conditioned problems e.g. the stack of cubes with a $10^4$ mass ratio presented in Figures 1 and 4.

\noindent
\reviewer{2.19} \citrev{It would be helpful to comment on the convexity of the NCP. 
Is Eq 27a convex? 
Is it challenging to solve because it is nonconvex or because of non-smoothness?}


\noindent
\response We thank the reviewer for this interesting question.
The problem (28a) is a convex QCQP.
This property appears to be useful because it allows the ADMM steps from (36a) and (36b) to be computed efficiently.
However, it is its coupling with equation (28b) through de Saxc`e correction that makes the NCP problem non-convex, non-smooth, and thus numerically hard.
In the revised manuscript, we added a comment on this point after introducing equation (28).

\noindent
\reviewer{2.20} \citrev{Eq 14, define H in positive semidefinite space of matrices}


\noindent
\response We thank the reviewer for pointing out this lack of precision.
We corrected this in the revised version.

\noindent
\reviewer{2.21} \citrev{Comment on the ADMM solver initialization and the ability to warmstart a physics step from the previous step.
How many iterations are required for a coldstart v warmstart?
}

\noindent
\response We thank the reviewer for this interesting comment.
Indeed, initializing a contact solver is not an easy task.
In our approach, we use the contact forces computed at the previous time step as a warm start whenever we are in a static scenario.
When this is the case, the ADMM solver converges immediately.
In the more general situation with moving contact points, our ADMM approach could benefit from its ability to handle infeasible guesses naturally.
For now, we use a zero initial guess, but finding a better guess is an open question that we leave for future work.

==> reviews/reviewers/reviewer-Tpqh.tex <==
\section{Reviewer Tpqh}

\subsection{Summary of limitations}


\noindent
\reviewer{4.1} \citrev{ [I] I didn't find any reference to the value of the time step Delta t used in the symplectic Euler integration scheme.
It would be extremely valuable for the reader to have access to this data to better assess the performance of the algorithm.
Being able to simulate large time steps robustly is a challenge.
It is known that the first order approximation made with the choice of an Euler integration scheme might result in unstable simulation with large time step.}

\noindent
\response We thank the reviewer for reporting this omission. 
We used a time step of 1ms for all our experiments which is specified in the revised paper at the beginning of the experiments in section V.A.
This choice allows to get a trade-off between simulation speed and solver reliability but we observe that our simulation remains stable for time steps below  30ms for the challenging wall of cubes scenario and up to 50ms for better conditioned problem such as UR5.
The inherent non-smoothness of the contact dynamics hinders the potential gain of using higher-order integration schemes.
Indeed, switching points in the dynamics e.g. the time instant when a contact occurs, degrades the integration orders and requires reduced time steps to be captured accurately \cite{studer2008step}.
However, evaluating the various integrators is an interesting research direction and would require its own dedicated study so we leave it as future work.

\noindent
\reviewer{4.2} \citrev{ [II] While I appreciate the benchmark comparisons with other solution methods (SCS, PGS) and problem formulation (convex relaxation: CCP), the authors could have included comparison with off-the-shelf solvers.
Indeed, the proposed baselines are not real/credible alternatives to the proposed approach.
The authors point out limitations of existing solvers like Drake and Mujoco in the introduction.
It would be great to provide some point of comparison to see how the proposed approach addresses these limitations.}

\noindent
\response Please see our response to the Area Chair's comment for more details on this point.

\noindent
\reviewer{4.3} \citrev{ [III] The authors could improve the quality of the work by providing insights into the failures modes of their proposed method. Understanding the failure modes and the root causes of these issues would provide invaluable information for the reader and could serve as a catalyst for driving future progress in the field.
It would be very interesting to see how often an din which scenarios the solver reaches the limit of ADMM steps (from the paper max iteration = 1e3) and returns a solution violating the constraint tolerances.}

\noindent
\response As mentioned in the paper, our solver currently does not have convergence guarantees just like other NCP solvers.
However, in practice, we observe that the solver often converges in a few iterations for robotics scenarios (Fig.3).
In the case of more complex mechanical systems, the approach may require a large number of iterations (see Fig.3 on the wall of cubes scenario) but still converges faster than current approaches (see Fig.3 and 5).
Therefore, it would be interesting in future works to investigate the potential convergence guarantees of the proposed algorithm.
We added this comment to the conclusion when evoking possible future works.

\noindent
\reviewer{4.4} \citrev{ [IV] The experiments related to the inverse dynamics method are quite limited. Given that the method is inspired from Todorov's work [1], it could be interesting to include evaluations of the inverse dynamics method similar to [1]. For instance in [1] Fig. 2, they compare the contact impulses obtained by forward dynamics and inverse dynamics. }

\noindent
\response We thank the reviewer for this suggestion.
In the revised paper we added figures similar to Fig.2 from \cite{6907751} comparing the contact forces computed by inverse and forward dynamics on UR5 experiment.
We observe that the contact forces computed by the inverse dynamics are consistent with the ones computed by the forward dynamics.
Please see our answer to 2.11 for more details on the efficiency of the contact inverse-dynamics algorithm.


\noindent
\reviewer{4.5} \citrev{Minor issues:
    typo b(q) <- b(q,v) after equation 1
    typo II.D routed <- rooted
    mu in Eq. 18 is overloaded with the friction coefficient
    table 1 Raisim and Dojo point to the same reference
    typo : missing parenthesis before "the minimizer of (47)."
    type: expalined <- explained}

\noindent
\response We thank the reviewer for reporting these typos.
We corrected them in the revised version of the paper.

\subsection{Feedback For Improvement Or Clarification:}


\noindent
\reviewer{4.6} \citrev{It would be very valuable if the authors could address these questions in the updated version of the manuscript.
[I]    What is the time step used for each problem?
    How sensitive to the time step size are the solution methods for both the forward dynamics and the inverse dynamics? in terms of solution times and solver robustness.
    Typically, what is the order of magnitude of the best time step size to trade off simulation speed and solver reliability?
    In Figures 3 and 4, the step size used in the Euler integration scheme is not explicitly stated. Investigating how these results evolve with different step sizes, including analyzing convergence rates and success, would be beneficial.
    Equation 22: It is proposed to evaluated the mass matrix and constraint Jacobians only once with the Euler symplectic scheme. What is the impact on stability, when is this an issue what kind of systems are made unstable by this simplification? In particular, linearizing the contact constraints at the current point can have a strong effect on systems with rolling contact, has this been observed in practice?}
    
\noindent
\response Please see R.4.1 for a discussion on the choice of time step and the impact on the stability of the simulation.

\noindent
\reviewer{4.7} \citrev{[II] It seems necessary to include comparison with off-the-shelf solvers to identify the differences in terms of solver accuracy (how much the convex relaxation impacts the solution), solve times, solver reliability (number of failures to converge to a solution).}

\noindent
\response Please see our response to the Area Chair's comment for more details on this point.

\noindent
\reviewer{4.8} \citrev{[III] What type of scenarios that are challenging for the proposed solver? large number of objects and collisions, impact between large and small objects, enforcing kinematic loops, etc.}

\noindent
\response Please see our response to R.4.3 for more details on this point.

\noindent
\reviewer{4.9} \citrev{What is the benefit of the update rule proposed in Eq. 45 vs the classical update rule in Eq. 43? The updates seems to be triggered by the same conditions and thus would results in the same number of update to the parameter rho.}

\noindent
\response As mentioned by the reviewer, the update rule proposed in Eq. 45 is triggered by the same conditions as the classical linear update rule in Eq. 43.
However, the proposed update rule is based on the spectral properties of the matrix G and the condition number is used to adapt $\rho$ which is not the case for the classical update rule.
This results in a lower number of updates and a more stable convergence.
Please see our answer to R.3.2 for an analysis of convergence rates.

\noindent
\reviewer{4.10} \citrev{In practice, what is the type of cones handled by the solver, is it using the second-order friction cone or the linearized friction cone? What are the tradeoffs there is terms of solver convergence for second-order cone vs linearized cone?}

\noindent
\response As mentioned in section II.E (equation 25) our approach considers second-order cones for friction.
Using second-order cones rather than pyramidal cones does not induce extra computational cost as the projection operations are of similar complexity.
Moreover, it is common to prefer second-order cones due to their isotropy and this choice is made in classical simulators e.g. MuJoCo, and Drake.

\noindent
\reviewer{4.11} \citrev{What is the effect of respecting Equation 4 instead of Equation 2. What are the benefits and drawbacks of this change on the numerical and physical standpoints?}

\noindent
\response We thank the reviewer for pointing out our evasive explanation on this point.
As mentioned just after Equation (4), proceeding to index reduction requires adding corrective terms to avoid the numerical drift of the original constraint. 
In the revised paper, we mention Baumgarte correction to be more precise on the type of correction we use.

\noindent
\reviewer{4.12} \citrev{The compliant constraints in Equation 6 generates a torque $tau_c$, should this be a wrench in general (if the system features, for instance, prismatic joints)?}

\noindent
\response For $\lambda$ we consider 3D contact forces rather than more general 6D wrenches. 
Then, applying the Jacobian transpose results in a torque in the configuration space.
We leave the extension to 6D wrenches as a future work.


==> reviews/reviewers/reviewer-b4hA.tex <==
\section{Reviewer b4hA}

\subsection{Summary of limitations}

\noindent
\reviewer{5.1} \citrev{ The main weakness of this paper is that the graphs are a little small and hard to read in the evaluation.
They could also be a bit better described to ensure that roboticists without as much background in contact dynamics can better understand the impact of the work and the importance of improving these kinds of software.}

\noindent
\response 
Additionally, as mentioned in R.2.2, the proposed approach could lead to accurate and computationally efficient robotics simulators that can run on CPUs.
We added a comment on this in the "Discussion" section by comparing our work to the recent advances related to MuJoCo XLA and Isaac Gym simulators.

\subsection{Feedback For Improvement Or Clarification:}

\noindent
\reviewer{5.2} \citrev{ As mentioned above, additional higher level clarifications of the impacts of the approach could be made in the evaluation and results section.
Deployments onto physical robots based on algorithms leveraging these improved contact models would also better validate the results and make the impact more clear to the broader community.}

\noindent
\response Please see 5.1 for a discussion on the potential impact of our approach.
We agree that deploying our approach on physical robots would allow us to confirm that accurate contact models are crucial for the success of robotic tasks.
Regarding the experimental effort this would require, we leave it for future work.
